Reducing Reparameterization Gradient Variance

Optimization with noisy gradients has become ubiquitous in statistics and machine learning. Reparameterization gradients, or gradient estimates computed via the "reparameterization trick," represent a class of noisy gradients often used in Monte Carlo variational inference (MCVI). However, when these gradient estimators are too noisy, the optimization procedure can be slow or fail to converge. One way to reduce noise is to use more samples for the gradient estimate, but this can be computationally expensive. Instead, we view the noisy gradient as a random variable, and form an inexpensive approximation of the generating procedure for the gradient sample. This approximation has high correlation with the noisy gradient by construction, making it a useful control variate for variance reduction. We demonstrate our approach on non-conjugate multi-level hierarchical models and a Bayesian neural net where we observed gradient variance reductions of multiple orders of magnitude (20-2,000x).

==> 3a_variance_analysis.tex <==
\section{Example}
\paragraph{Linear approximations} 
More generally, $\tilde \bff$ in Equation~\ref{eq:data-term-approx} can be viewed as a linear approximation of the data term gradient as a function of $\epsilon$.
In fact, we can choose any linear approximation
\begin{align}
	\tilde \bff &= \bbeta_0 + \bbeta \epsilon 
\end{align}
parameterized by $\bbeta_0 \in \mathbb{R}^D$ and $\bbeta \in \mathbb{R}^{D \times D}$ (or a more constrained diagonal $\bbeta$).

To use this type of linear approximation, we must first determine appropriate values of $\bbeta_0$ and $\bbeta$. 
In Equation~\ref{eq:data-term-approx} we used the gradient and the hessian of the log-likelihood term evaluated at $\bmm_\blambda$.
However, if the dimensionality of the posterior $D$ is too large, the Hessian will be computationally intractable. 
Even though we can efficiently generate samples by computing a Hessian-vector product with $\epsilon$ (which does not cost much more than 2-3 function evaluations), to this as a control variate requires that we characterize the scale parameter of the distribution, which corresponds to the diagonal of the Hessian. 
The diagonal of the Hessian is not efficiently computable --- a naive method would be require essentially $D$ function evaluations, which is computationally prohibitive for larger models.

Given this restriction, there are other ways to set these parameters given multiple samples drawn at each iteration, $L$.  
\begin{itemize}
	\item \emph{Independent least squares}: we can regress the values $\hat \bff^{(\ell)}$ on $\epsilon^{(\ell)}$, independently by dimension (e.g.~$\bbeta$ is diagonal)
	\item \emph{Multivariate Least Squares}: we can do the same regression as above, but with a full $\bbeta$ --- this will be $\mathcal{O}(D^3)$
	\item \emph{Low Rank or Random Projection Least Squares}: do the same regression as above, but use a low rank $\bbeta$ matrix.
	\item \emph{Approximate Hessian Diagonal}: we can approximate the diagonal of the Hessian (e.g.~Becker+Le Cun, Ilya's paper, trace approx)
	\item \emph{Full Hessian}: use the full Hessian if computable.
\end{itemize}

\todo[inline]{How much ``noise'' is introduced when we start using sample-based estimators within each step?  Where does increased efficiency come from, if any?}

\todo[inline]{render a figure showing the relationship between $\epsilon$ and $\hat \bff(\bz)$}

\todo[inline]{compare the residuals + correlation of Full Hessian vs Approx Diag}


\paragraph{Sample-based estimators}


\begin{figure}[t!]
\includegraphics[width=\textwidth]{../figs/data_term_fig/epsilon_vs_gsample-model-frisk.pdf}
\caption{Base noise vs gradient samples along eight dimensions of an example model posterior.  Note that, even though $\hat \bg(\epsilon)$ is a deterministic function, interaction between dimensions creates what looks like irreducible noise when regressing along a single dimension.  From these visualizations, we can infer that the independent least squares regressors will have a wide range of irreducible variance.}
\end{figure}



%To this end, we approximate the distribution of $f(\bz)$ by the delta method, based on the first-order Taylor approximation
%\begin{align}
%& \bz \sim \mathcal{N}(\bmm_\blambda, \bs_\blambda^2) \\
%& f_\blambda(\bz) \\
%&\approx f_{\blambda}(\bmm_\blambda) + f'_{\blambda}(\bmm_\blambda)(\bz - \bmm_\blambda) \\
%%&\triangleq \tilde f_{\blambda}(\bmm_\blambda).
%&\sim \mathcal{N}\left(\tilde \bmm_{\blambda}, \tilde \bs_{\blambda}^2 \right)
%&=       f_{\blambda}(\bmm_\blambda) + f'_{\blambda}(\bmm_\blambda)((\epsilon \cdot \bs_\blambda + \bmm_\blambda) - \bmm_\blambda) \\
%\end{align}
%where we have defined parameters 
%\begin{align}
%    \tilde \bmm_{\blambda} &\triangleq f_{\blambda}(\bmm_\blambda) \\
%    \tilde \bs_{\blambda} &\triangleq f'_{\blambda}(\bmm_\blambda) s_\blambda.
%\end{align}

%We use $f'_{\blambda}$ to denote the derivative of the gradient of $\ln p(\bz, \mathcal{D})$ at location $\blambda$ (which $\bz$ depends on).
%We note that this is not necessarily the Hessian, as we may consider each dimension independently when the dimension of the posterior $D$ is large.\footnote{Though we consider individual elements of the gradient independently, we can use the full Jacobian to construct a richer, though more expensive approximation.}

%Applying the gradient of the log probability function to a random variate $\bz$ is a transformation of a Gaussian.
%The locally linear approximation of the transformation allows the result to be approximated with another Gaussian. 

%Given this approximation for the model gradient term's distribution, we can characterize the distribution for the variational parameter gradient for the mean and variance ($m_\blambda$ and $s_\blambda$).
%\begin{align}
%\frac{\partial \mathcal{L}}{m_\blambda} 
%	&\sim \mathcal{N}(m_{\blambda, p}, s_{\blambda,p}^2) 
%\end{align}
%and 
%\begin{align}
%\frac{\partial \mathcal{L}}{s_\blambda} 
%	&\sim (m_{\blambda, p} + s_{\blambda,p} z_0) \cdot z_0 + 1/s_\blambda
%\end{align}
%The expectation of the standard deviation parameter gradient is 
%\begin{align}
%\mathbb{E}\left[\frac{\partial \mathcal{L}}{s_\blambda}\right]
%	&= s_{\blambda, p} + 1/s_\blambda 
%\end{align}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\columnwidth]{../figs/plot_gradient_marginals_and_approx_out/iter-10-baseball-dlnp_dz_delta_approx_no_hessian.pdf}
        \caption{Iteration 10}
        \label{fig:iter-10}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{.45\textwidth}
        \includegraphics[width=\columnwidth]{../figs/plot_gradient_marginals_and_approx_out/iter-50-baseball-dlnp_dz_delta_approx_no_hessian.pdf}
        \caption{Iteration 50}
        \label{fig:iter-50}
    \end{subfigure}
\caption{Comparison of true samples of the data term and the Gaussian approximation for 8 dimensions of a hierarchical model.  The blue histogram reflect 1000 true samples of the data term.  The green pdf is the delta-method based Gaussian approximation. }
\label{fig:data-term-approx}
\end{figure}

Figure~\ref{fig:data-term-approx} depicts our approximation of the distribution of the data term for a selection of marginals of the posterior of a hierarchical model.
The top shows the approximation early in the optimization procedure, which is generally quite accurate.
The bottom figure shows the approximation after 50 iterations of ELBO optimization, and we see that the approximation deteriorates somewhat due to the non-Gaussianity of the posterior. 
While the distributional accuracy of this approximation is desirable, it is the correlation between $\hat \bg_\blambda$ and $\tilde \bg_\blambda$ that matters most. 

%We empirically explore our delta-method approximation to the gradient distribution in Figure~\ref{fig:baseball-data-distribution}.
%We can see that the approximation is more accurate earlier on in the optimization procedure (particularly if we initialize with low variance).  
%\begin{itemize}
%\item To be ``black box'', we have to approximate the transformation due to the data model 
%\end{itemize}

